Voltage Stability and Control of Electrical Distribution Systems with High Penetration of Power Electronic Converters

Power systems are currently undergoing a rapid paradigm change in their operation. Centralised energy production is being replaced by a number of Distributed Generation (DG) units that are placed at different locations and voltage levels in power networks. These distributed units are mostly based on renewable energy technologies, like wind turbines and photovoltaic cells and are commonly interfaced to the grid via power electronic converters. These sources reduce energy system dependency on conventional generation units based on fossil fuels. At the same time, this shift introduces technical challenges for the safe and reliable operation of electricity network since DG sources do not inherently provide the grid regulation services of conventional, centralised generation units. Moreover, the increased penetration of renewable energy sources and their converter-based interfaces is creating voltage deviation and voltage stability issues in distribution networks. These issues range from overvoltages during hours of peak renewable generation, reverse power flows and sudden voltage drops due to the variable nature of renewable energy production. All of the above jeopardise the reliable operation of the distribution networks that were not originally designed to accommodate for these effects. The objective of this thesis is to propose novel techniques for the accurate assessment of the DG impact on voltage stability in distribution net works and investigate how the control capabilities of converter-based interfaces of DG units can be harnessed to improve stability margins and overall system robustness and performance.

==> Deposito.tex <==

\thispagestyle{empty}

\cleardoublepage

\includepdf[pages=1]{ImagenesCover/Registro.pdf}

\thispagestyle{empty}

==> ch_papers.tex <==


\thispagestyle{empty}

\cleardoublepage

\includepdf[pages=-]{PDF_Papers/J1_Bifurcation}

\thispagestyle{empty}

\cleardoublepage

\includepdf[pages=-]{PDF_Papers/C1_VAL.pdf}

\thispagestyle{empty}

\cleardoublepage

\includepdf[pages=-]{PDF_Papers/C2_QVAL.pdf}

\thispagestyle{empty}

\cleardoublepage

\includepdf[pages=-]{PDF_Papers/J2_Recursive_QVAL.pdf}

\thispagestyle{empty}

\cleardoublepage

\includepdf[pages=-]{PDF_Papers/J3_Taxonomy.pdf}

\thispagestyle{empty}

\cleardoublepage

\thispagestyle{empty}

